TokenPilot: Cache-Efficient Context Management for LLM Agents

As LLM agents are deployed in long-horizon sessions, context accumulation drives up inference costs. Existing approaches utilize text pruning or dynamic memory eviction to minimize token footprints; however, their unconstrained sequence mutations alter layouts, introducing prefix mismatches and cache invalidation. This reveals a critical trade-off between text sparsity and prompt cache continuity. To address this, we present TokenPilot, a dual-granularity context management framework. Globally, Ingestion-Aware Compaction acts as a framework harness to stabilize prompt prefixes and eliminate open-world environmental noise at the ingestion gate. Locally, Lifecycle-Aware Eviction monitors the ongoing residual utility of context segments, enforcing a conservative batch-turn schedule to offload content segments only when task relevance expires. Experiments on PinchBench and Claw-Eval under both isolated and continuous modes demonstrate that TokenPilot reduces costs by 61% and 56% in isolated mode, and 61% and 87% in continuous mode, while maintaining competitive performance compared to prior systems. TokenPilot has been integrated into LightRSI at https://github.com/zjunlp/RSI.

==> table/claw-eval_isolated.tex <==
\definecolor{VanillaColor}{RGB}{235,235,235}
\definecolor{StaticCompressionColor}{RGB}{255,228,225}
\definecolor{OursColor}{RGB}{235,225,245} 
\begin{table}[t]
\centering
{\setlength{\tabcolsep}{10pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|cc|ccc}
\toprule[1pt]
\textbf{Method} & \textbf{Overall $\uparrow$} & \textbf{Cost (\$) $\downarrow$} & \textbf{Cache Read (M)} & \textbf{Cache Miss (M)} & \textbf{Output (M)} \\
\midrule
\rowcolor{VanillaColor} Vanilla          &           &           &           &           &           \\
\rowcolor{StaticCompressionColor} LLMLingua-2      &           &            &           &           &           \\
\rowcolor{StaticCompressionColor} SelectiveContext  &           &            &           &           &           \\
\rowcolor{OursColor} \textbf{TokenPilot}       & 49.06          & 3.07           &  5.322         &  2.061         &  0.250         \\
\bottomrule[1pt]
\end{tabular}
}}
\caption{Ablation Comparison with Pre-history Processing in \texttt{Claw-Eval}. \textbf{Best results} in bold.}
\label{tab:claw-eval_isolated}
\end{table}
